Physical Inertial Poser (PIP): Physics-aware Real-time Human Motion Tracking from Sparse Inertial Sensors

Motion capture from sparse inertial sensors has shown great potential compared to image-based approaches since occlusions do not lead to a reduced tracking quality and the recording space is not restricted to be within the viewing frustum of the camera. However, capturing the motion and global position only from a sparse set of inertial sensors is inherently ambiguous and challenging. In consequence, recent state-of-the-art methods can barely handle very long period motions, and unrealistic artifacts are common due to the unawareness of physical constraints. To this end, we present the first method which combines a neural kinematics estimator and a physics-aware motion optimizer to track body motions with only 6 inertial sensors. The kinematics module first regresses the motion status as a reference, and then the physics module refines the motion to satisfy the physical constraints. Experiments demonstrate a clear improvement over the state of the art in terms of capture accuracy, temporal stability, and physical correctness.

==> sec/experiments/livedemo.tex <==
We perform some live demos to further demonstrate the power of our system.
%
More live results are shown in our supplementary video.
\XY{TODO}

==> sec/method/notations.tex <==
\noindent\textbf{Reference Frame.}\XY{here}
%
In our method, we use 2 different coordinate systems to describe body motion for different sub-tasks:
%
\textit{1)} the local system which is relative to the root joint of human;
%
and \textit{2)} the global system that keeps static.
%
The transformation between these two systems composes a rotation matrix and a translation vector.
%
The rotation can be directly read from the IMU mounted on the root joint, and the translation is estimated by our method as explained later.
%
%----------------------------------------------------------------------------------
%
\par\noindent\textbf{Physics Model.}
%
We use a torque-controlled floating-base character as our physical model \cite{Zheng2013}\XY{here}, and follow the same mass distribution as in \cite{PhysCap}.
%
Since the IMUs do not provide any positional measurement, we initialize the subject's global position at the origin.
%
We refer to the joint positions in the global system as $\boldsymbol r$ and the translation as $\boldsymbol r_{\mathrm{root}}$.
%
The time derivative $\dot{\boldsymbol r}$ and $\ddot{\boldsymbol r}$ refer to linear velocity and acceleration, respectively.
%
The joint rotations are referred as $\boldsymbol \theta$, which is also called \textit{pose} parameters.
%
The time derivative $\dot{\boldsymbol \theta}$ and $\ddot{\boldsymbol \theta}$ are the joint angular velocity and acceleration, respectively.
%
The configuration of the character can be described by its pose and translation, which we denote as $\boldsymbol q=[\boldsymbol r_{\mathrm{root}}\,\,\,\,\boldsymbol \theta] \in \mathbb{R}^N$ where $N=3+3J$ is the degree of freedom (DoF) of the character.
%
The time derivative $\dot{\boldsymbol q}$ and $\ddot{\boldsymbol q}$ are the generalized velocity and acceleration of the model.
%
The character is controlled by the vector of force $\boldsymbol \tau \in \mathbb{R}^N$ where each dimension refers to the force on the corresponding DoF.
%
In the real world, the character is actuated only by the torques at the $J-1$ non-root joints, while no force is applied to the root joint itself.
%
However, to compensate the dynamics mismatch between our physical model and real humans \cite{ResidualForceControl}, we allow a small residual force at the unactuated root joint, following previous works \cite{PhysCap,ResidualForceControl,PhysAware,SimPoE,PhysSimulationLevine2012}.
%
In our notation, the first six entries $\boldsymbol \tau_{:6}$ correspond to the residual force at the root joint, and $\boldsymbol \tau_{6:}$ are the actuated joint torques.
%
The generalized acceleration $\ddot{\boldsymbol q}$ and force $\boldsymbol \tau$ follow the equation of motion \cite{RigidBodyDynamics}:
%
\begin{equation}
    \boldsymbol \tau + \boldsymbol J(\boldsymbol q)^T\boldsymbol \lambda = \boldsymbol M(\boldsymbol q)\ddot{\boldsymbol q} + \boldsymbol h(\boldsymbol q, \dot{\boldsymbol q}),
\end{equation}
%
where $\boldsymbol M \in \mathbb{R}^{N \times N}$ is the inertia matrix;
%
$\boldsymbol h \in \mathbb{R}^N$ is the non-linear effect term that accounts for gravity, Coriolis, and centripetal forces;
%
$\boldsymbol \lambda \in \mathbb{R}^{3n_c}$ is the external contact force applied at $n_c$ contact points on the physical character;
and $\boldsymbol J \in \mathbb{R}^{3n_c \times N}$ is the contact point Jacobian\XY{here} that maps the generalized velocity of the model to the contact point velocities:
%
\begin{equation} \label{eq:Jqdot}
    \dot{\boldsymbol r} = \boldsymbol J \dot{\boldsymbol q}.
\end{equation}
%
Readers are referred to \cite{RigidBodyDynamics} for more details.
%
In our model, we assume all external contact forces come from supporting and friction forces from the ground, which we call \textit{ground reaction force (GRF)}.
%
\begin{comment}
%
%----------------------------------------------------------------------------------
%
\par\noindent\textbf{Inputs.}
%
The raw inputs are the acceleration and orientation measurements of the 6 IMUs.
%
Before tracking, our method performs a fast T-pose calibration as in \cite{TransPose}.
%
We denote the calibrated accelerations as $\boldsymbol a_1 \cdots \boldsymbol a_6 \in \mathbb{R}^3$ and the orientations as $\boldsymbol R_1 \cdots \boldsymbol R_6 \in \mathbb{R}^{3 \times 3}$.
%
For the root joint we directly use the orientation and acceleration retrieved from the sensor, while for other joints we compute the root-relative measurements.
%
The concatenated vector $\boldsymbol x=[\hat{\boldsymbol a}_1 \cdots \hat{\boldsymbol a}_6\,\,\,\,\hat{\boldsymbol R}_1 \cdots \hat{\boldsymbol R}_6] \in \mathbb{R}^{72}$ forms our inputs.
%
%---------------------------------------------------------------------------
%
\par\noindent\textbf{Outputs.}
%
The outputs of the system are the pose $\boldsymbol \theta$, the translation $\boldsymbol r_\mathrm{root}$, the ground reaction force $\boldsymbol \lambda$, and the torques at each joint $\boldsymbol \tau$.
\end{comment}
